Recovering boundary conditions in inverse Sturm-Liouville problems

We introduce a variational algorithm, which solves the classical inverse Sturm-Liouville problem when two spectra are given. In contrast to other approaches, it recovers the potential as well as the boundary conditions without a priori knowledge of the mean of the potential. Numerical examples show that the algorithm works quite reliable, even in the presence of noise. A proof of the absence of strict local minimizers of the functional supports the observation, that a good initial guess is not essential.

==> gnuplothead.tex <==
\ifx\PSTloaded\undefined
\def\PSTloaded{t}
\psset{arrowsize=.01 3.2 1.4 .3}
\psset{dotsize=.01}
\catcode`@=11

\newpsobject{PST@Border}{psline}{linewidth=.01,linestyle=solid}
\newpsobject{PST@Axes}{psline}{linewidth=.01,linestyle=dotted,dotsep=.004}
\newpsobject{PST@Solid}{psline}{linewidth=.015,linestyle=solid}
\newpsobject{PST@Dotted}{psline}{linewidth=.01,linestyle=dashed,dash=.05 .05}%{psline}{linewidth=.01,linestyle=dashed,dash=.05 .05}
\newpsobject{PST@Dashed}{psline}{linewidth=.012,linestyle=dotted,dotsep=.01}
%\newpsobject{PST@LongDash}{psline}{linewidth=.012,linestyle=dashed,dash=.02 .01}
\newpsobject{PST@LongDash}{psline}{linewidth=.01,linestyle=dashed,dash=.05 .05}
\newpsobject{PST@Diamond}{psdots}{linewidth=0.3,dotsize=0.025,dotscale=1,dotstyle=square,linestyle=solid,dotangle=45}
\newpsobject{PST@Filldiamond}{psdots}{linewidth=.001,linestyle=solid,dotstyle=square*,dotangle=45}
\newpsobject{PST@Cross}{psdots}{linewidth=.001,linestyle=solid,dotstyle=+,dotangle=45}
\newpsobject{PST@Plus}{psdots}{linewidth=.001,linestyle=solid,dotstyle=+}
\newpsobject{PST@Square}{psdots}{linewidth=.001,linestyle=solid,dotstyle=square}
\newpsobject{PST@Circle}{psdots}{linewidth=.001,linestyle=solid,dotstyle=o}
\newpsobject{PST@Triangle}{psdots}{linewidth=.001,linestyle=solid,dotstyle=triangle}
\newpsobject{PST@Pentagon}{psdots}{linewidth=.001,linestyle=solid,dotstyle=pentagon}
\newpsobject{PST@Fillsquare}{psdots}{linewidth=.001,linestyle=solid,dotstyle=square*}
\newpsobject{PST@Fillcircle}{psdots}{linewidth=.001,linestyle=solid,dotstyle=*}
\newpsobject{PST@Filltriangle}{psdots}{linewidth=.001,linestyle=solid,dotstyle=triangle*}
\newpsobject{PST@Fillpentagon}{psdots}{linewidth=.001,linestyle=solid,dotstyle=pentagon*}
\newpsobject{PST@Arrow}{psline}{linewidth=.001,linestyle=solid}
\catcode`@=12

\fi

